Evaluation of Portable Acceleration Solutions for LArTPC Simulation Using Wire-Cell Toolkit

The Liquid Argon Time Projection Chamber (LArTPC) technology plays an essential role in many current and future neutrino experiments. Accurate and fast simulation is critical to developing efficient analysis algorithms and precise physics model projections. The speed of simulation becomes more important as Deep Learning algorithms are getting more widely used in LArTPC analysis and their training requires a large simulated dataset. Heterogeneous computing is an efficient way to delegate computing-heavy tasks to specialized hardware. However, as the landscape of the compute accelerators is evolving fast, it becomes more and more difficult to manually adapt the code constantly to the latest hardware or software environments. A solution which is portable to multiple hardware architectures while not substantially compromising performance would be very beneficial, especially for long-term projects such as the LArTPC simulations. In search of a portable, scalable and maintainable software solution for LArTPC simulations, we have started to explore high-level portable programming frameworks that support several hardware backends. In this paper, we will present our experience porting the LArTPC simulation code in the Wire-Cell toolkit to NVIDIA GPUs, first with the CUDA programming model and then with a portable library called Kokkos. Preliminary performance results on NVIDIA V100 GPUs and multi-core CPUs will be presented, followed by a discussion of the factors affecting the performance and plans for future improvements.

==> kokkos-rng.tex <==
\subsection{Kokkos random number generator}
\label{subsec-kokkos-rng}




==> sigproc.tex <==
\subsection{Signal Processing Module}
\textcolor{red}{Do we want to include this? Perhaps we should concentrate on the sim module in this paper - ML}

Since the data processed in this module is signals of constant size, each signal is represented by a row vector and the signals are represented by a matrix.
The most time consuming part is the filtering followed by the inverse discrete Fourier transformation (DFT) and sorting (to compute median value of the signal) for signals.
The signals are discretized  by $6000$ grids and the number of signals is 800 $\sim$ 960.
Listing \ref{list:before} shows C++ source code of the filtering followed by the inverse DFT.
Since the basic computation unit is one signal (one row), the example of the profiling needs 800 $\sim$ 900 inverse DFT of vector of 6000 length after the filtering. 

\begin{lstlisting}[language={C++}, 
caption={Original source code part converted to CUDA.},
basicstyle=\ttfamily\footnotesize,
label={list:before}]
Array::array_xxc c_data_afterfilter(m_c_data.rows(), m_c_data.cols());
for (int irow = 0; irow < m_c_data.rows(); ++irow) {
  for (int icol = 0; icol < m_c_data.cols(); ++icol) {
    c_data_afterfilter(irow, icol) =
      m_c_data(irow, icol) * roi_hf_filter_wf.at(icol);
  }
}
Array::array_xxf tm_r_data = Array::idft_cr(c_data_afterfilter, 0);
m_r_data = tm_r_data.block(m_pad_nwires[plane], 0, m_nwires[plane], m_nticks);
\end{lstlisting}

As a test-bed, we applied CUDA acceleration on that part.
The code part of Listing \ref{list:before}  takes about 13.43\% of whole running time (77.1381 / 574.446).
The speed-up after CUDA acceleration is summarized in Table \ref{table:speedup1}.
The accelerated part (Listing \ref{list:before}) shows about 18 times speed-up.
The overall speed-up is $14 \%$.
The time measurement of GPU code (after CUDA acceleration) includes data transfer time between CPU memory and GPU memory.
A CUDA kernel function is implemented for the filtering and cuFFT is called for the inverse DFT.



\begin{table}[ht]
\begin{center}
\begin{tabular}{c || c | c}
    \hline
Running time (sec) & Accelerated Part & Whole Code \\
    \hline\hline
    
CPU & 77.1381 & 574.446 \\ \hline
GPU & 4.20504 & 502.203 \\ \hline 
Speed-up & 18.34  & 1.14 \\ \hline 

\hline
\end{tabular}
\caption{Simulation running times of CPU code and GPU acceleration. This test is conducted on Intel Xeon\textsuperscript{\textregistered} CPU E5-2695 v4 @ 2.10 GHz and NVIDIA Tesla P100.}
\label{table:speedup1}
\end{center}
\end{table}

==> wct.tex <==
\section{LArTPC Simulation with Wire-Cell Toolkit - Haiwang/Brett}
\label{sec-wct}

Current CPU Oriented implementation in \wct.
% alg. description
% Advantage of WC 2D sim
